Benchmarking the Performance and Energy Efficiency of AI Accelerators for AI Training

Deep learning has become widely used in complex AI applications. Yet, training a deep neural network (DNNs) model requires a considerable amount of calculations, long running time, and much energy. Nowadays, many-core AI accelerators (e.g., GPUs and TPUs) are designed to improve the performance of AI training. However, processors from different vendors perform dissimilarly in terms of performance and energy consumption. To investigate the differences among several popular off-the-shelf processors (i.e., Intel CPU, NVIDIA GPU, AMD GPU, and Google TPU) in training DNNs, we carry out a comprehensive empirical study on the performance and energy efficiency of these processors by benchmarking a representative set of deep learning workloads, including computation-intensive operations, classical convolutional neural networks (CNNs), recurrent neural networks (LSTM), Deep Speech 2, and Transformer. Different from the existing end-to-end benchmarks which only present the training time, We try to investigate the impact of hardware, vendor's software library, and deep learning framework on the performance and energy consumption of AI training. Our evaluation methods and results not only provide an informative guide for end-users to select proper AI accelerators, but also expose some opportunities for the hardware vendors to improve their software library.

==> sec7.tex <==
\section{Discussion: More AI Accelerators} \label{sec:dc}
% AI accelerators
There are also accelerators offered by various vendors that are not officially included in our benchmark. For instance, Ascend 910 processor released by Huawei under Da Vinci Architecture delivers up to 256 TFLOPS FP16 under the maximum power of 310W. Huawei has also developed MindSpore computation framework that best fits the Ascend processors. 

Another AI Accelerator that has achieved state-of-the art performance in many Deep Learning training tasks is the Intelligence Processing Unit (IPU) processor provided by Graphcore. The IPU is designed for parallel computation of sparse high dimensional graphs and data structures\cite{kacher2020graphcore}. IPU supports both DNN training and inference. Instead of focusing on training or inference, it focus instead on hardware that can support continuous learning in the core or at the edge of the network \cite{jia2019dissecting}. It is built on the understanding of properties of deep learning workloads including the parallelism, the sparsity and the statistical approximation. To better scatter and gather data, it is designed to have more processors to process smaller vectors than GPUs. To avoid the limitations in performance of DNN workloads brought by the bandwidth of external DRAM, Graphcore adopts SRAM only in IPU for a memory-centric chip - in which way, the limitations of applications that are bottle-necked by latency in small bandwidth is largely reduced. However, the radical approach has also raised some challenges brought by the shrinking of memory capacity compared with GPUs and TPUs. Graphcore has provided some solutions for that - when the model is too big, there are multi-chip interconnection and model parallelism mechanism to deal with the lack of memory. The training pipeline also introduces re-computation to trade computation for memory with Bulk Synchronous Parallel (BSP) approach. 

A Graphcore C2 card contains two IPUs, the maximum power of which are 300w in total. One IPU is built with large core counts of 1216 IPU-Cores. 256kB of on-chip memory is coupled to each IPU core, adding up to 304MB of SRAM memory. The memory bandwidth is up to 45TBps thanks to the design. We use Graphcore’s Poplar SDK to program with IPU. The functions in Poplar are well optimized for IPU, similar to CUDA for NVIDIA GPUs. Due to the architectural distinctions, the benchmark of IPU is not included in our metrics. However, we would still like to talk about the characteristics of IPU to explore the development direction of future AI Accelerators.


\begin{table}[htbp]
  \centering
  \caption{The comparison of IPU, GPU and TPU’s performance (FLOPS) and utilization of the Matmul operator. (Left: TFLOPS; Right: Utilization)}
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
    \toprule
    Matmul & \multicolumn{2}{c|}{IPU(FP16)} & \multicolumn{2}{c|}{IPU(FP32)} & \multicolumn{2}{c|}{V100(TC)} & \multicolumn{2}{c|}{V100(FP32)} & \multicolumn{2}{c|}{TPU-v2(bfloat16)} \\
    \midrule
    \midrule
    1024*1024 & 42.87 & 34.43\% & 16.38 & 52.67\% & 79.51 & 70.99\% & 12.16 & 86.06\% & 142.28 & 79.04\% \\
    \midrule
    2048*2048 & 43.31 & 34.79\% & 16.92 & 54.41\% & 82.88 & 74.00\% & 12.87 & 91.08\% & 167.94 & 93.30\% \\
    \bottomrule
    \end{tabular}%
  \label{tab:ipu}%
\end{table}%

We conduct experiments on Azure IPU with Poplar SDK version 1.1.11. The Graphcore IPU is featured in a Microsoft Azure instance as the NDv3. NDv3 VMs feature eight Graphcore C2 IPU-Processor PCIe Cards, with 16 Graphcore IPUs. An NDv3 VM also includes 40 cores of CPU, backed by Intel Xeon Platinum 8168 processors and 768 GB of memory, and 4TB of fast NVMe scratch disk. Most of the experimental settings in our benchmark do not fit IPU because IPU does not support large batch sizes. However, we still manage to conduct the same benchmark on the performance of small Matmul ops with Poplar SDK on IPU, in comparison with other AI accelerators. As can be seen from Table \ref{tab:ipu}, when dealing with small Matmul ops that fully utilizes the SRAM on IPU chips, IPU-core make less use of the parallelism of calculations than V100 and TPU v2. The reason lies in that the IPU core processes calculations more granular than V100 TensorCores and TPU cores, limited by the port of maximum 128 bit for IPU-core accessing the local SRAM. 

Still, IPU surpasses GPU in quite a few DNN tasks. For example, IPU delivers 1.25$\times$ higher performance than V100 on Resnext-50 with model parallelism, as well as from 4$\times$ up to >100$\times$ performance in Group Convolution Kernels. IPU has also shown great advantages in many other training tasks including reinforcement learning, time series analysis, and so on. The high performance of IPU in many workloads based on the unique hardware design and a perfected software environment has made Graphcore a strong challenger to giant vendors like Intel, NVIDIA, Google, and Huawei.































